ImPoster: Text and Frequency Guidance for Subject Driven Action Personalization using Diffusion Models

We present ImPoster, a novel algorithm for generating a target image of a 'source' subject performing a 'driving' action. The inputs to our algorithm are a single pair of a source image with the subject that we wish to edit and a driving image with a subject of an arbitrary class performing the driving action, along with the text descriptions of the two images. Our approach is completely unsupervised and does not require any access to additional annotations like keypoints or pose. Our approach builds on a pretrained text-to-image latent diffusion model and learns the characteristics of the source and the driving image by finetuning the diffusion model for a small number of iterations. At inference time, ImPoster performs step-wise text prompting i.e. it denoises by first moving in the direction of the image manifold corresponding to the driving image followed by the direction of the image manifold corresponding to the text description of the desired target image. We propose a novel diffusion guidance formulation, image frequency guidance, to steer the generation towards the manifold of the source subject and the driving action at every step of the inference denoising. Our frequency guidance formulations are derived from the frequency domain properties of images. We extensively evaluate ImPoster on a diverse set of source-driving image pairs to demonstrate improvements over baselines. To the best of our knowledge, ImPoster is the first approach towards achieving both subject-driven as well as action-driven image personalization. Code and data is available at https://github.com/divyakraman/ImPosterDiffusion2024.

==> Figures/table2.tex <==
\begin{table*}
    \centering
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule 
        Method & CLIP & DINO & SSCD & Phase \\
        \midrule 
        Textual Inversion~\cite{gal2022image} (ICLR 2023) & $0.2861$ &	$0.3123$ &	$0.2243$ &	$0.7512$ \\
Dream Distribution~\cite{zhao2023dreamdistribution} (arXiv 2023)	& $0.2832$ &	$0.3521$ &	$0.2122$ & 	$0.7502$ \\
T2I Adapter~\cite{mou2024t2i} (arXiv 2023)	& $0.2810$ &	$0.3422$ &	$0.2911$ &	$0.7501$ \\
ADI~\cite{huang2024learning} (CVPR 2024)	& $0.2998$&	$0.2933$ &	$0.2666$ &	$0.7495$ \\
Fast Composer~\cite{xiao2023fastcomposer} (IJCV 2024)	& $0.2765$ &	$0.3453$ &	$0.2461$ &	$0.7502$ \\
Baseline++ (inspired by DreamBooth LoRA and Custom Diffusion, CVPR 2023) & $0.2897$ &	$0.5538$ &	$0.4517$ &	$0.7515$ \\
ImPoster	& $0.3055$ &	$0.3665$ &	$0.2903$ &	$0.7529$ \\
       \bottomrule
    \end{tabular}
    }
    %\vspace*{-0.5em}
    \caption{\textbf{More state-of-the-art comparisons.} Comparisons against textual inversion variants (Textual Inversion, DreamDistribution), subject-driven approaches (FastComposer, Baseline++), ControlNet variants (T2I adapter) and action customization approaches (ADI) reveal that ImPoster is able to successfully transfer the driving motion while retaining the characteristics of the source subject, and achieves a better trade-off between driving action (CLIP/Phase score) and source subject (SSCD/DINO) than prior work. }
    %\vspace*{-1.5em}
    \label{tab:metrics}
\end{table*}


==> Sections/0-abstract.tex <==
\begin{abstract}
    We present ImPoster, a novel algorithm for generating a target image of a `source' subject performing a `driving' action. The inputs to our algorithm are a single pair of a source image with the subject that we wish to edit and a driving image with a subject of an arbitrary class performing the driving action, along with the text descriptions of the two images. Our approach is completely unsupervised and does not require any access to additional annotations like keypoints or pose. Our approach builds on a pretrained text-to-image latent diffusion model and learns the characteristics of the source and the driving image by finetuning the diffusion model for a small number of iterations. At inference time, ImPoster performs \emph{step-wise text prompting} i.e. it denoises by first moving in the direction of the image manifold corresponding to the driving image followed by the direction of the image manifold corresponding to the text description of the desired target image. We propose a novel diffusion guidance formulation, \emph{image frequency guidance}, to steer the generation towards the manifold of the source subject and the driving action at every step of the inference denoising. Our frequency guidance formulations are derived from the frequency domain properties of images. We extensively evaluate ImPoster on a diverse set of source-driving image pairs to demonstrate improvements over baselines. To the best of our knowledge, ImPoster is the first approach towards achieving both subject-driven as well as action-driven image personalization. We will make all code and data publicly available.  
\end{abstract}

\begin{figure*}   
    \centering
    \includegraphics[scale=0.27]{Figures/coverPic.jpg}
    \caption{\textit{Given a single ``source'' image and a ``single'' driving image and the corresponding text descriptions, ImPoster generates an image of the source subject performing driving action.} We show how ImPoster is able to make a monkey and an alien meditate and play violin.}
    \label{fig:teaser}
    %\vspace{-10pt}
\end{figure*}

% Remove: SOTA table; Modify: User study    

==> macros.tex <==
%\newcommand{\rohan}[1]{\textcolor{red}{#1}}
\newcommand{\bigO}[1]{\mathcal{O}(#1)}
\newcommand{\sota}{state-of-the-art}
%\newcommand{\trisha}[1]{\textcolor{red}{#1}}
%\newcommand{\utt}[1]{\textcolor{blue}{#1}}
\newcommand{\tian}[1]{\textcolor{orange}{#1}}
\newcommand{\divya}[1]{\textcolor{blue}{#1}}
\newcommand{\model}{BlackScholesDiff}
\newcommand{\datanames}{Sub-$k$ matrices}
% \newcommand{\sota}{state-of-the-art}
\newcommand{\G}{$G$}
\newcommand{\V}{$V$}
%\newcommand{\E}{$E$}
\newcommand{\brr}[1]{\left( #1 \right)}
\newcommand{\bcc}[1]{ \left{ #1 \right} }
\newcommand{\bss}[1]{\left[ #1 \right]}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\sg}{\mathcal{L}}
\newcommand{\li}{\sg}
\newcommand{\vts}[1]{\lvert #1 \rvert}
\newcommand{\Vts}[1]{\lVert #1 \rVert}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand\inv[1]{#1\raisebox{1.05ex}{$\scriptscriptstyle-\!1$}}
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-1.3ex]{0pt}{0pt}}   % = `bottom' strut
\newcommand\Bstrutfrac{\rule[-0.7ex]{0pt}{0pt}}   % = `bottom' strut
\newcommand\Tstrutfrac{\rule{0pt}{1.7ex}}         % = `top' strut
\newcommand\mathdash{\text{\normalfont --}}
\newcommand{\cost}{\bigO{ \vts{\li^{\scriptscriptstyle -1}_t}k }}
\newcommand{\cm}{\mathcal{M}_{\Delta t}(u)}
\newcommand{\pc}{\zeta_c(t)}
\newcommand{\pd}{\zeta_d(t)}
\newcommand{\pe}{\zeta_e(t)}
\newcommand{\costk}{\bigO{ \vts{\li^{\scriptscriptstyle -1}_t} }}
\newcommand\setrow[1]{\gdef\rowmac{#1}#1\ignorespaces}
% \newcommand{\cost}{\bigO{\vts{\delta} \vts{\mc{L}_{i_{\vts{\mc{I}_{\delta}}}}}^2 }}
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother
\newcommand{\size}{\bigO{d}}
\newcommand{\shorteq}{%
  \settowidth{\@tempdima}{-}% Width of hyphen
  \resizebox{\@tempdima}{\height}{=}%
}
\newcommand*\midpoint[1]{\overline{#1}}
% \renewcommand{\thefootnote}{\fnsymbol{footnote}}
\newcommand{\mysetminus}{\mathbin{\fgebackslash}}

% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% \usepackage[noend]{algpseudocode}
\let\proof\relax
\let\endproof\relax

%\setlength{\parskip}{-0.1em}
\mathchardef\mhyphen="2D

\newcommand{\minus}{\scalebox{0.75}[1.0]{$-$}}

\definecolor{RowColorCode}{rgb}{0.61,0.57,0.89}

%\linespread{0.988}
